Nonparametric Hamiltonian Monte Carlo

Probabilistic programming uses programs to express generative models whose posterior probability is then computed by built-in inference engines. A challenging goal is to develop general purpose inference algorithms that work out-of-the-box for arbitrary programs in a universal probabilistic programming language (PPL). The densities defined by such programs, which may use stochastic branching and recursion, are (in general) nonparametric, in the sense that they correspond to models on an infinite-dimensional parameter space. However standard inference algorithms, such as the Hamiltonian Monte Carlo (HMC) algorithm, target distributions with a fixed number of parameters. This paper introduces the Nonparametric Hamiltonian Monte Carlo (NP-HMC) algorithm which generalises HMC to nonparametric models. Inputs to NP-HMC are a new class of measurable functions called "tree representable", which serve as a language-independent representation of the density functions of probabilistic programs in a universal PPL. We provide a correctness proof of NP-HMC, and empirically demonstrate significant performance improvements over existing approaches on several nonparametric examples.

==> 5experiments.tex <==
% !TEX root = ./main.tex

We implemented the NP-HMC algorithm and its variants (NP-RHMC and NP-DHMC) in Python, using PyTorch \cite{pytorch} for automatic differentiation.
In our empirical evaluation, we focus on the NP-DHMC algorithm because it inherits discontinuous HMC's efficient handling of discontinuities:
contrary to NP-RHMC, it does not need to compute the intersections of the particle's trajectory with the regions of discontinuity.
Our implementation also uses the efficiency improvements discussed at the end of \cref{sec:np-hmc}.

We compare our implementation with inference algorithms that are applicable out-of-the-box to nonparametric models:
importance sampling (IS), Metropolis-Hastings (MH) with proposal kernel described in \cite{DBLP:conf/icfp/BorgstromLGS16} and a corrected version of Lightweight Metropolis-Hastings (LMH) \cite{DBLP:journals/jmlr/WingateSG11}, on
the following probabilistic programs with an unbounded number of random variables.

%\lo{Isn't the algorithm in \cite{HurNRS15} a version of LMH?}
%\cm{No, the proposal sample is obtained by sampling a new value for each element in the current sample.}

\begin{table}
\begin{center}
\footnotesize
\caption{Total variational distance from the ground truth for the geometric distribution. Averaged over 10 runs, each run with $10^3$ samples, $10^2$ burn-in, 5 leapfrog steps of size 0.1.}
\label{table:geometric-tvd}
\vspace{0.1in}
\begin{tabular}{lllll}
\toprule
method &\textbf{ours} &IS &MH &LMH \\
\midrule
TVD &\textbf{0.0139} &0.0152 &0.2382 &0.0251 \\
\bottomrule
\end{tabular}
\end{center}
\end{table}

\paragraph{Geometric distribution}
A classic example to illustrate recursion in a universal PPL is sampling from a geometric distribution with parameter $p$ by repeatedly flipping a biased coin with probability $p$ (see e.g.~Ch.~5 in \cite{intro-prob-prog}).
The pseudocode for it is:
\begin{minipage}{\columnwidth}
\begin{python}
def geometric():
  if sample(uniform(0, 1)) < p: return 1
  else: return 1 + geometric()
\end{python}
\end{minipage}
We tested our algorithm on this problem with $p = 0.2$.
Our implementation works well on this example and has no trouble jumping between traces of different length.
To quantify this, we computed the total variational distance to the ground truth for each approach and report it in \cref{table:geometric-tvd}.
The result is perhaps surprising given that the odds are ``stacked against'' NP-DHMC in this model:
it is a discrete model, so there is no gradient information, and there are no observations (only sampling from the prior).
These properties should favour importance sampling and LMH, making the performance of NP-DHMC rather remarkable.

%\paragraph{Infinite Gaussian mixture \& function induction}
%In addition, we considered two examples from \cite{DBLP:conf/icml/ZhouYTR20}: a Gaussian mixture model with a random number of components and function induction.
%In both cases, NP-HMC struggles to transition from one configuration to another, a problem it shares with many other MCMC algorithms \cite{DBLP:conf/icml/ZhouYTR20}.
%For instance, in the Gaussian mixture, it never switches to a different number of mixture components.

%\anon{LAFI R2: Could it be because it is difficult for MCMC to jump between modes (is that what you mean by “configurations”?). Perhaps reducing the distance between the modes in the prior / generated data, would help with this and would allow you to evaluate NP-HMC without being constrained by this problem (as the problem applies more fundamentally to MCMC and is tangential to this work).}

%\anon{Zhou: In terms of examples, I think the open GMM from DCC paper is actually a great choice. The poisson prior on K fits nicely for the tree structure. I am interested to see why it does not transit. Have you had a look of the trace plot of K and mus, from different iid runs.

%HMC is very sensitive to trajectory length and step size as well. Take the GMM case, you might need different L and epsilon to work well restricted to different K. However, I am not sure this is allowed in HMC or not.

%If we forget about transition among different traces/Ks, does your HMC algorithm converge correctly within the chosen K?}

%\anon{Zhou: The latter part of this sentence is a bit misleading. I am sure you are referring to the discussions about the failure of existing MCMC methods in DCC paper. However, it reads like DCC is the one that cannot transit, whereas DCC is proposed to solve this problem.

%This is just a minor rewording point :) }

\paragraph{Random walk}
To better evaluate our algorithm on probabilistic programs with unbounded loops (such as the example from \cref{sec:tr-functions}), we considered the one-sided random walk on $\pReal$ described in \cite{MakOPW20}:
A pedestrian starts from a random point in $[0,3]$ and walks a uniformly random distance of at most 1 in either direction, until they pass 0.
Given a (noisily) measured total distance of 1.1 travelled, what is the posterior distribution of the starting point?
As this process has infinite expected running time, we need a stopping condition if the pedestrian is too far away from zero, (\pythoninline{distance < 10}), as shown in the following pseudocode:
\begin{python}
start = sample(uniform(0,3))
position = start; distance = 0
while position > 0 and distance < 10:
  step = sample(uniform(-1, 1))
  position += step; distance += abs(step)
observe(distance, normal(1.1, 0.1))
return start
\end{python}

\begin{figure}[h!]
\centering
\footnotesize
\includegraphics[width=\columnwidth]{img/walk-kde.pdf}
\begin{tabular}{lllll}
\toprule
method &\textbf{ours} &IS &MH &LMH \\
\midrule
ESS &\textbf{7131.0} &439.2 &647.7 &74.0 \\
\bottomrule
\end{tabular}
\caption{Kernel density estimate (top) averaged over 10 runs and estimated effective sample size (bottom) computed using 10 runs (1000 samples each, burn-in: $100$, HMC step size: 0.1; leapfrog steps: 50).}
\label{fig:walk}
\end{figure}
% \paragraph{Random walk}
% To better evaluate our algorithm on probabilistic programs with unbounded loops (such as the example from \cref{sec:tr-functions}), we considered the one-sided random walk example on $\pReal$ described in \citet{MakOPW20}:
% A pedestrian starts on a uniformly random point of $[0,3]$ and walks a uniformly random distance of at most 1 in either direction, until they pass 0.
% Given a (noisily) measured total distance of 1.1 travelled, what is the posterior distribution of the starting point?
% As this process has infinite expected running time, we need a stopping condition if we're too far away from zero, as shown in the following pseudocode (\pythoninline{distance < 10}):
% \begin{python}
% start = sample(uniform(0,3))
% position = start; distance = 0
% while position > 0 and distance < 10:
%   step = sample(uniform(-1, 1))
%   position += step; distance += abs(step)
% observe(distance, normal(1.1, 0.1))
% return start
% \end{python}

The results are shown in \cref{fig:walk}.
The sampled posterior distribution is consistent with and less noisy than importance sampling.
This example is interesting and challenging because the true posterior is difficult to determine precisely.
Therefore we took $10^7$ importance samples (effective sample size $\approx 4.4 \times 10^5$) and consider this as the ground truth.
As one can see from \cref{fig:walk}, NP-DHMC comes closest.
Since it is not clear what measure to use for the distance from these ``ground truth'' samples, we instead computed the effective sample size\footnote{We used the standard ESS estimator (based on weighted samples) for the IS samples, and an autocorrelation-based MCMC ESS estimator (Sec.~11.5 in \cite{Gelman2014}) for the rest. However the latter estimator gives a similar result (469.0) on the IS samples, so the two ESS estimators are comparable in this case.}
%\footnote{For IS one would use an ESS estimator based on weighted samples. However, the MCMC ESS estimator (which is based on autocorelation \cite{vehtari2020rank}) applied to the IS samples gives a similar result (469.0), so the numbers should still be comparable.}
for each method (\cref{fig:walk}).
Our method does best in that regard as well.

\begin{figure}
\centering
\includegraphics[width=\columnwidth]{img/walk-pyro-kde.pdf}
\vspace{0.1in}
\vspace{-0.3in}
\caption{Kernel density estimate for the random walk example compared to Pyro, averaged over 10 runs (1000 samples each, burn-in: $100$, HMC step size: 0.1; leapfrog steps: 50).}
\label{fig:walk-pyro}
\end{figure}
\changed[lo]{The popular PPL Pyro accepts nonparametric models as input.
%Therefore, we thought it would be interesting \changed[cm]{to see} how Pyro's HMC implementation performs on this example.
We therefore tried to ascertain the performance of its HMC implementation on this example.}
We ran both Pyro's HMC sampler (with the same hyperparameters as ours for this example) and Pyro's No-U-Turn sampler (NUTS) \cite{HoffmanG14}, which aims to automatically infer good hyperparameter settings.
%Pyro's inference was very slow, sometimes taking almost a minute to produce a single sample.
%The inferred posterior distributions (\cref{fig:walk-pyro}) are also far away from the ground truth, and clearly wrong.
The inferred posterior distributions (\cref{fig:walk-pyro}) are far away from the ground truth, and clearly wrong.
Pyro’s inference was very slow, sometimes taking almost a minute to produce a single sample.
\changed[lo]{For this reason, we didn't run more experiments with it.}



%This gives further justification to NP-HMC, seeing as standard HMC implementation struggle with this example.
\fz{Let me know what you think about this. Also, does the plot take up too much space?}
\cm{I wonder if we could add the Pyro plots to Fig 5. Don't worry if it's too crowded. Another note about colours. I think it would be nice to use a different colour for the Pyro engines and keep the colour of ground truth consistent with Fig 5.}
\fz{I can do it, but I think it would be too crowded.}

\begin{figure}
\centering
\includegraphics[width=\columnwidth]{img/gmm-histogram.pdf}
\vspace{0.1in}
\vspace{-0.3in}
\caption{Histogram of the no.~of mixtures for the GMM example; correct posterior = 9. Averaged over 10 runs with 1000 samples; burn-in: 100, HMC step size: 0.05; leapfrog steps: 50.}
\label{fig:gmm}
\end{figure}
\begin{table*}
\centering
\caption{Log pointwise predictive density (LPPD) for the Gaussian mixture model (GMM) and the Dirichlet Process Mixture Model (DPMM) , mean and standard deviation from 10 runs. Each GMM run: samples: 1000, burn-in: 100, leapfrog steps 50, step size: 0.05. Each DPMM run: samples: 100, burn-in: 50, leapfrog steps 20, step size: 0.05.}
\vspace{0.1in}
\begin{tabular}{lllllll}
\toprule
model &``true'' &\textbf{ours} &IS &MH &LMH \\
\midrule
GMM &-674.81 &$\mathbf{-675.64 \pm 0.47}$ &$-743.40 \pm 10.96$ &$-765.86 \pm 16.25$ &$-729.59 \pm 11.55$ \\
DPMM &-674.81 &$\mathbf{-677.53 \pm 0.49}$ &$-743.88 \pm 11.16$ &n/a &$-740.28 \pm 9.72$ \\
\bottomrule
\end{tabular}
\label{table:gmm-lppd}
\end{table*}
\paragraph{Gaussian mixture model}
We also considered the following mixture model adapted from \cite{DBLP:conf/icml/ZhouYTR20}, where the number of mixture components $K$ is unbounded.
\begin{align*}
K &\sim \mathrm{Poisson}(10) + 1 \\
\mu_k &\sim \mathrm{Uniform}([0, 100]^3) &&\text{for } k = 1,\dots,K \\
x_n &\sim \frac{1}{K}\sum_{k=1}^K \Gau_3(\mu_k, 10^2I_3) &&\text{for } n = 1,\dots,N
\end{align*}
This model samples parameters $\theta = (K\in \Nat, \mu_k \in [0,100]^3)$ and $N$ data points $X = \{x_1,\dots,x_N\} \subseteq \Real^3$.
Note that this model uses much higher standard deviations (10 instead of 0.1) for the Gaussian mixture components compared to \cite{DBLP:conf/icml/ZhouYTR20}.
This is to avoid typical problems of MCMC algorithms with multimodal distributions, which is an issue inherent to MCMC algorithms and tangential to this work.
We used this model to generate $N = 200$ training data points for a fixed $\theta^* = (K^* = 9, \mu_{1\dots K^*}^*)$.
We let our inference algorithms sample from $p(\theta \mid X)$ and compared the posterior on the number of mixture components $K$ with the other inference algorithms.
The histogram (\cref{fig:gmm}) shows that NP-DHMC usually finds the correct number of mixture components ($K^* = 9$), whereas the other algorithms infer a number that is too high.

In addition, we computed the log pointwise predictive density (LPPD) for a test set with $N' = 50$ data points $Y = \{y_1,\dots,y_{N'}\}$, generated from the same $\theta^*$ as the training data.
The LPPD is defined as $\sum_{i=1}^{N'} \log \int p(y_i \mid \theta) p(\theta \mid X) \dif\theta$ and can be approximated by $\sum_{i=1}^{N'} \log \frac{1}{M} \sum_{j=1}^M p(y_i \mid \theta_j)$ where $(\theta_j)_{j=1\dots M}$ are samples from $p(\theta \mid X)$ \cite{Gelman2014}.
The results (\cref{table:gmm-lppd}) include the ``true'' LPPD of the test data under the point estimate $\theta^*$.
As we can see, NP-DHMC outperforms the other methods and has the lowest variance over multiple runs.

\paragraph{Dirichlet process mixture model}
Finally, we consider a classic example of nonparametric models: the Dirichlet process $\mathrm{DP}(\alpha, H)$ \cite{Ferguson73}, which is a stochastic process parametrised by concentration parameter $\alpha > 0$ and a probability distribution $H$.
For practical purposes, one can think of samples from $\mathrm{DP}(\alpha, H)$ as an infinite sequence $(w_k, h_k)_{n\in \Nat}$ where $w_n$ are weights that sum to 1 and $h_n$ are samples from $H$.
Conceptually, a DP Gaussian mixture model takes the form
\begin{align*}
(w_k, h_k)_{k\in \Nat} &\sim \mathrm{DP}(\alpha, H) \\
x_n &\sim \sum_{k=1}^\infty w_k \cdot \Gau(h_k, \Sigma) &&\text{for } n = 1,\dots,N
\end{align*}
Sampling from a DP is usually implemented by the stick-breaking method \cite{Sethuraman94}.
However, one cannot actually compute an infinite sequence.
A practical workaround is to cap the number of mixture components by a fixed $K$ and only consider $(w_k, h_k)_{k=1,\dots,K}$.%\footnote{See, for example, the Pyro tutorial on DP mixture models: \url{https://pyro.ai/examples/dirichlet_process_mixture.html}. Accessed: 2021-2-4.}
\footnote{For instance, see \url{https://pyro.ai/examples/dirichlet_process_mixture.html} (accessed: 2021-2-4), the Pyro tutorial on DP mixture models.}
%This makes the model parametric again, facilitating the use of standard HMC.
%However, if the data actually requires more mixture components than $K$, such a model will be insufficient.
\changed[lo]{This renders the model parametric, enabling the use of standard HMC.
However such a treatment is clearly unsatisfactory: if the data actually requires more mixture components than $K$, the model would be found wanting.}


We propose a different approach.
Instead of choosing a fixed $K$, we allow it to depend on the weights $w_k$:
we pick the minimal $K \in \Nat$ such that $\sum_{i=1}^K w_i > 1 - \epsilon$ for some $\epsilon > 0$.
With this restriction, we only discard insignificant mixture components (with a weight $w_k < \epsilon$) and allow as many mixture components as necessary to model the data accurately.
This model is not parametric anymore, but still tractable by our algorithm.

We implemented the above model with the parameters $\alpha = 5$, $\epsilon = 0.01$, and the remaining parameters as chosen in the previous GMM example, i.e.~$H = \mathrm{Uniform}([0,100]^3)$ and $\Sigma = 10^2I_3$.
We used the same training and test data as in the previous GMM example and report the LPPD in \cref{table:gmm-lppd}.
Our algorithm clearly performs the best.
Note that MH failed to produce samples in a reasonable amount of time, so it was excluded.


==> prettyplots.tex <==
% !TEX root = ./main.tex

\begin{tikzpicture}
\begin{axis}[
    axis lines = left,
    xlabel = $\vec{q}_1$,
    ylabel = {Energy},
    xmin=-4, xmax=4,
    ymin=0
]
% red plot
\addplot [
  domain=-4:0,
  samples=100,
  color=red,
]
{-ln(1/sqrt(2*pi)*exp(-(1/2)*x^2))};
\addlegendentry{$-\log(\phi(0\mid \vec{q}_1,1))\cdot [\vec{q}_1 \leq 0]$}
% points on red plot
\node[label={45:{[-3.1]}},circle,fill,inner sep=2pt] at (axis cs:-3.1,5.72393853) {};
\node[label={45:{[-2.37]}},circle,fill,inner sep=2pt] at (axis cs:-2.37,3.72738853) {};
\node[label={45:{[-0.86]}},circle,fill,inner sep=2pt] at (axis cs:-0.86,1.28873853) {};
\end{axis}
\end{tikzpicture}

\begin{tikzpicture}
  \begin{axis}[
    axis lines = left,
    xlabel = $\vec{q}_1$,
    ylabel = $\vec{q}_2$,
    zlabel = {Energy},
    xmin=-4, xmax=4,
    ymin=-4, ymax=4,
    zmin=0,
    view={15}{5},
  ]
  % red plot
  \addplot3 [
    mesh,
    domain=-4:0,
    y domain=-4:4,
    samples=20,
    color=red,
  ]
  {-ln(1/sqrt(2*pi)*exp(-(1/2)*x^2))};
  \addlegendentry{$-\log(\phi(0\mid \vec{q}_1,1))\cdot [\vec{q}_1 \leq 0]$}
  % points on red plot
  \node[label={[fill=white, fill opacity=0.6, text opacity=1]90:{[-3.1, -2]}},circle,fill,inner sep=2pt] at (axis cs:-3.1,-2,5.72393853) {};
  \node[label={[fill=white, fill opacity=0.6, text opacity=1]90:{[-2.37, -0.9]}},circle,fill,inner sep=2pt] at (axis cs:-2.37,-0.9,3.72738853) {};
  \node[label={[fill=white, fill opacity=0.6, text opacity=1]90:{[-0.86, 0.2]}},circle,fill,inner sep=2pt] at (axis cs:-0.86,0.2,1.28873853) {};

  % blue plot
  \addplot3 [
    mesh,
    domain=0:4,
    y domain=0:4,
    restrict z to domain=0:8,
    samples=20,
    color=blue
  ]{(y > x) ? -ln(1/sqrt(2*pi)*exp(-(1/2)*(y-x)^2)):-1};
  \addlegendentry{$-\log(\phi(\vec{q}_2\mid \vec{q}_1,1))\cdot [0 < \vec{q}_1 \leq \vec{q}_2]$}
  % points on blue plot
  \node[label={[fill=white, fill opacity=0.6, text opacity=1]45:{[1.15, 1.3]}},circle,fill,inner sep=2pt] at (axis cs:1.15,1.3,0.930188533) {};
  \end{axis}
\end{tikzpicture}
